Interpretable Representation via LLM-Driven Generative Disentanglement for Local-Life Service Recommendation

While large language models (LLMs) have advanced ID-based recommendation through Semantic ID (SID) modeling, existing SID generation frameworks largely follow a single-representation-then-quantization paradigm. This design faces two bottlenecks: semantic entanglement mixes heterogeneous attributes, such as geography, brand, and category, causing information loss during quantization, low-quality SIDs, and severe collisions; moreover, black-box representation learning provides neither explicit attribute semantics nor clear geographic or semantic meanings for SID positions. These limitations weaken both retrieval reliability and the ability to diagnose or control SID generation. We propose Interpretable Representation via LLM-Driven Generative Disentanglement for Local-Life Service Recommendation (LGRID). LGRID introduces a generative disentanglement paradigm through an Encode -> Disentangle -> Align -> Quantize pipeline. It first uses joint LLM encoding to preserve cross-attribute geographic-semantic dependencies, rather than encoding fields independently. A Structured Disentangled Block then routes hidden states into attribute-aligned slots for geographic and semantic factors. Synergistic Alignment Learning makes these slots both generatively decodable and discriminative for retrieval, while Dual-Stream Residual Quantization separately discretizes the two streams into compact SIDs with explicit attribute correspondence. This design yields interpretable SIDs with positions grounded in item attributes and local-service semantics. Experiments on Kuaishou and Foursquare show that LGRID consistently outperforms strong SID baselines, achieving up to a 5.44 percent relative AUC gain. It also achieves over 99 percent attribute-decoding accuracy for coarse geographic fields and reduces the full-SID collision rate to 39.9 percent, compared with 97.0 percent for LGSID.

==> resubmission_summary.tex <==
% KDD 2027 resubmission summary. This material must occupy exactly one page.
\begingroup
\onecolumn
\thispagestyle{empty}
\normalsize
\setlist[itemize]{leftmargin=1.15em,itemsep=0.10em,topsep=0.10em,parsep=0pt,partopsep=0pt}

\begin{center}
  {\Large\bfseries Summary of Changes}
\end{center}

\noindent
We revised the manuscript in response to each concern raised in the previous
KDD reviews. Each bullet below corresponds to one reviewer comment and briefly
summarizes the change now reflected in the paper.

\noindent\textbf{Reviewer rDPk.}
\begin{itemize}
  \item \textbf{On what is new beyond LGSID.} We agree that the distinction
  needed to be made explicit. We now explain that LGSID strengthens a single
  geo-enhanced item embedding, whereas LGRID first preserves geo--content
  dependencies through joint LLM encoding and then separates them into
  LLM-decodable geographic and semantic slots before dual-stream residual
  quantization, as shown in the Abstract (p.1), Introduction (pp.1--2),
  Related Work--Item Tokenization (p.2), and Appendix B.2/Table 12 (pp.12--13).
  \item \textbf{On whether the distance threshold $D$ is fixed.} We clarified
  that $D$ defines a spatially valid candidate set rather than a modeling
  assumption of LGRID. The revised protocol states that Kuaishou uses a fixed
  offline $D=15$ km threshold only for LGSID-comparable benchmarking, while
  Foursquare follows full ranking because no production distance policy is
  available, as shown in Problem Definition (p.3) and Appendix A.3 (p.12).
  \item \textbf{On the domain-specific prompt tokens in Eq.~(1).} We now state
  that the initial slot tokens $\mathbf{Z}^{(0)}$ are initialized from eight
  semantic anchors corresponding to physical POI attributes, rather than from
  answer-bearing prompts. The exact anchor phrases and robustness check are
  given in Semantic Anchor Injection (p.4), Appendix B.1/Table 11 (p.12), and
  Appendix C.4/Table 18 (p.15).
  \item \textbf{On the runtime comparison with RQ-VAE.} We added a direct
  efficiency analysis showing that LGRID's extra cost is offline SID
  construction (21.80 vs. 13.97 ms/item), while online input preparation remains
  nearly unchanged (0.50 vs. 0.48 ms/request). This is reported in
  Experiment--Efficiency (p.8) and Appendix A.4/Table 10 (p.12).
\end{itemize}

\noindent\textbf{Reviewer SLhp.}
\begin{itemize}
  \item \textbf{On why disentanglement is needed when structured fields exist.}
  We added a field-wise structured-encoding baseline to test this alternative
  directly. The new results show that independent field encoding loses useful
  geo--content interactions, while joint encoding followed by structural
  decoupling improves all six attribute-retrieval dimensions, as discussed in
  the Introduction (p.2), Joint LLM Encoding (p.3), Table 4 (p.6), the Joint
  encoding necessity analysis (p.7), and Appendix C.1/Table 16 (p.14).
  \item \textbf{On the implementation of baselines with SIDs.} We revised the
  method and appendix to make the fusion rule reproducible: for non-SID
  recommenders, the four SID-code embeddings are summed and concatenated with
  the original item-ID embedding, and all methods share the same split,
  candidate set, and evaluation labels. This is described in Deployment and
  Pipeline Summary/Algorithm 1 (p.5) and Appendix A.2--A.3 (pp.11--12).
  \item \textbf{On codebook collision rates.} We added full-SID collision and
  prefix-utilization analyses because item distinguishability is central to SID
  quality. The revised manuscript reports that LGRID reduces collision to
  39.9\%, compared with 98.0\% for RQ-VAE and 97.0\% for LGSID, as shown in the
  Abstract (p.1), SID collision analysis/Table 5 (p.7), and Appendix C.2
  (pp.14--15).
\end{itemize}

\noindent\textbf{Reviewer pu4u.}
\begin{itemize}
  \item \textbf{On the effectiveness of the loss terms in Eq.~(13).} We added
  direct removals of $\mathcal{L}_{\mathrm{PGD}}$,
  $\mathcal{L}_{\mathrm{SACL}}$, and $\mathcal{L}_{\mathrm{LDR}}$, together with
  component-level ablations, to show how decodability, discrimination, and
  slot diversity contribute separately. These results appear in Synergistic
  Alignment Learning (pp.4--5), Ablation Study/Tables 6--7 (pp.7--8), and
  Appendix C.3/Table 17 (p.15).
  \item \textbf{On source code, model weights, and reproducibility.} We expanded
  the release and reproducibility details rather than leaving the complex
  framework under-specified. The revised appendix gives dataset statistics, the
  120k/5k POI-text split, filtering rules, $K=6$ hard negatives, LoRA schedule,
  hyperparameters, hardware, and downstream recommendation settings, as shown
  in the Abstract footnote (p.1) and Appendix A.1--A.2 (pp.11--12).
  \item \textbf{On the confusing methodology pipeline.} We reorganized the
  method around the actual construction order--encode $\to$ disentangle $\to$
  align $\to$ quantize--so the modules are no longer presented as a stack of
  disconnected components. The revised flow is stated in Overview (p.3),
  Algorithm 1 and Deployment and Pipeline Summary (p.5).
\end{itemize}

\noindent\textbf{Reviewer kPRk.}
\begin{itemize}
  \item \textbf{On missing ablations for LGRID submodules.} We expanded the
  ablation section beyond the original SD-Block variants to cover SCR, SACL
  sampling, $\mathcal{L}_{\mathrm{PGD}}$, $\mathcal{L}_{\mathrm{SACL}}$, and
  $\mathcal{L}_{\mathrm{LDR}}$. The added results show which failure mode each
  component addresses, as reported in Ablation Study/Tables 6--7 (pp.7--8),
  Appendix B.4--B.5 (pp.13--14), and Appendix C.3/Table 17 (p.15).
  \item \textbf{On the design of PGD, CoT prompts, and SFT tasks.} We rewrote
  PGD as seven instruction--slot--answer supervised fine-tuning tasks, with
  explicit slot ranges, conditioning context, target fields, prompts, and loss
  masks. The main mechanism is described in PGD (p.4), and the complete task
  schema and prompts are given in Appendix B.3/Tables 13--15 (pp.12--14).
  \item \textbf{On the actual LGRID pipeline.} We made the end-to-end pipeline
  explicit from construction to downstream use: LGRID jointly encodes POI text,
  disentangles slots with SD-Block, aligns them with PGD/SACL/LDR, quantizes
  geographic and semantic streams separately, and fuses the resulting SIDs with
  recommender backbones. This is summarized in Overview (p.3), Algorithm 1 and
  Deployment and Pipeline Summary (p.5), and Appendix B.6 (p.14).
\end{itemize}

\clearpage
\endgroup

